ISEEQ: Information Seeking Question Generation using Dynamic Meta-Information Retrieval and Knowledge Graphs

Conversational Information Seeking (CIS) is a relatively new research area within conversational AI that attempts to seek information from end-users in order to understand and satisfy users' needs. If realized, such a system has far-reaching benefits in the real world; for example, a CIS system can assist clinicians in pre-screening or triaging patients in healthcare. A key open sub-problem in CIS that remains unaddressed in the literature is generating Information Seeking Questions (ISQs) based on a short initial query from the end-user. To address this open problem, we propose Information SEEking Question generator (ISEEQ), a novel approach for generating ISQs from just a short user query, given a large text corpus relevant to the user query. Firstly, ISEEQ uses a knowledge graph to enrich the user query. Secondly, ISEEQ uses the knowledge-enriched query to retrieve relevant context passages to ask coherent ISQs adhering to a conceptual flow. Thirdly, ISEEQ introduces a new deep generative-adversarial reinforcement learning-based approach for generating ISQs. We show that ISEEQ can generate high-quality ISQs to promote the development of CIS agents. ISEEQ significantly outperforms comparable baselines on five ISQ evaluation metrics across four datasets having user queries from diverse domains. Further, we argue that ISEEQ is transferable across domains for generating ISQs, as it shows the acceptable performance when trained and tested on different pairs of domains. The qualitative human evaluation confirms ISEEQ-generated ISQs are comparable in quality to human-generated questions and outperform the best comparable baseline.

==> dump.tex <==
% conversation information seeking, its challenges and our problem directions
% research on conversational models of information seeking hasbeen hampered by the lack of reusable datasets.
% We focus on a curiosity-driven, information-seeking scenario where a user starts a conversation with an assistant by asking an open-ended question and then drills down into interest areas
% Example of blockchain 
% More gen-erally,  systems  for  conversational  information-seeking should help users develop their informationneed, be mixed-initiative, incorporate user memory,and reason about the utility of retrieved informa-tion as a combined set
%  Talk about crowdsourcing as the limitation -- ISEEQ is efficient
% you can briefly explain the crowdsourcing scenario
% properties of the question from ppt -- paper from lehnert, schank etc.

Information Seeking is evident from people performing Google searches or using any online platform, such as Reddit or Twitter. Likewise, clinical interviews involve information-seeking behavior from the clinician. There are three main ways people seek information: 
\begin{enumerate}
    \item  \texttt{Title and Description}: \\
           Title: I am feeling down and depressed \\
Description: I am going through a rough patch in my life. With divorce proceedings and poor growth at work, I am feeling low and hopeless. What do you advise?
    \item \texttt{High-level Topic and Aspects }\\
 High-level topic: It seems Anxiety\\
 Aspects: Panic Attacks, trauma, relationship life
 \item \texttt{Description only }\\
Description: Not sure what is happening with me, but I am losing control of myself and taking XX meds and YY treatments. It seems nothing is working for me. I have other health conditions.
\end{enumerate}

In such situations, a google search would map the user query to pre-existing queries from other users to support you with 
"People Also Ask" or "Search Engine Results Page" (SERP) questions. However, an expert human would try to map the user's query condition to: (a) Cover high-level topics, (b) Tailored to user-specific topics, and (c) Context-switch to cover parallel but related information. Such a process characterizes a human's ability to learn and exhibit information-seeking behavior. Recent studies promote conversational information-seeking (CIS) systems \cite{zamani2020macaw} or conversational assistance (CA) systems, a sub-field within open domain question answering (ODQA) to enhance conversational artificial intelligence. However, the methods focus on improving information retrieval, either by query rewriting or passage ranking, rather than facilitating a dialog \cite{yu2020few}\cite{dalton2020cast}. Certainly, CIS/CA raises the standard in ODQA by developing datasets (a) that contain questions with no direct answer and (b) require explicit knowledge for generating questions that preserve context and are driven by curiosity (manifestation of a user's information-seeking behavior). Existing factoid question answering and goal-oriented question answering systems fall short in generating information-seeking questions necessary for conversational assistance with a user\cite{gao2018neural}. Studies on clarifying question generation and follow-up question generation differ because they explore the context provided by the user through description and input questions (see Figure 1).  \cite{rodriguez2020information} also acknowledge that CIS/CA differs from past question generation systems and requires an approach driven by curiosity over the user's input question. 

We expand the field of CIS and CA by presenting a novel pipeline of knowledge-aware passage retriever and conceptual-flow-based question generations conditioned over three properties: (a) Semantic relations between questions, (b) A logical agreement defining the conceptual flow, and (c) Legibility of question in terms of grammar and semantic meaning.
Our pipeline exploits transformer language models by placing them in a generative adversarial framework and optimized based on reward and entailment conditions.  The structure of our framework inherits the characteristics of information-seeking question generation systems, which are conceptually outlined in \cite{lehnert1977process}, \cite{schank1977rules}, \cite{van1987assumptions}, \cite{graesser2008question}. Specifically, in this research, we ask the following questions:
\begin{enumerate}
    \item Can we develop a method that generates a sequence of information-seeking questions, given an input query?
    \item Can common-sense knowledge and contextual entities from the user's input help in effective passage retrieving and question generation?
    \item Can we generate questions that are semantically related and entailed to have a conceptual flow?
    \item How do we evaluate such a method? 
\end{enumerate}

To address these challenges, we leverage conversational discourse datasets that fall into two categories: (a) Given a user query, questions have entailment; (b) Given a user query, questions have semantic relations between them; (c) Given a user query, questions have free form  For (a), we considered Conversation Assistance Track Dataset (CAsT-19) \cite{dalton2020cast}, and Facebook Curiosity Dataset \cite{rodriguez2020information}.  For (b), we considered Question Answering Discourse (QADiscourse) Dataset \cite{pyatkin2020qadiscourse}, and Question Answer Meaning Representation (QAMR) Dataset \cite{michael2018crowdsourcing}. 
One major challenge was the structure of these datasets which do not align with our problem statement. These datasets were created for different tasks, such as dialog act classification, question type classification, passage ranking, fact verification, and others. We reorient and semantically process these datasets for our purpose and outline the process before we apply our approach and baselines. For our problem statement, there are no prior approaches that can act as baselines. Hence, we fine-tune the state-of-the-art transformer models that are (a) either a part of these open-source datasets or (b) have shown to perform competitively in question answering.  We first evaluate the performance of our passage retriever on the QAMR dataset and then question generator on QAMR, QADiscourse, CAsT-19, and Facebook Curiosity. We decided to test the retriever on QAMR because of the noisiness of passages in Wikinews. 

\begin{table*}[t]
\footnotesize
\begin{center}
\begin{tabular}{p{5.4cm}|p{5.4cm}|p{5.4cm}}
    \toprule[1.5pt]
      \multicolumn{3}{c}{\textbf{Input:} What to know about 
David Mcletchie from Scottish 
Conservative party?} \\ \midrule[1pt]
      \textbf{Clarifying Questions} & \textbf{Follow-up Questions} & \textbf{Information Seeking} \\ \midrule
      Who is David Mcletchie? & Who is David Mcletchie? & What is the reason he was a former 
leader of the Scottish Conservatives? \\
What is a Conservative Party? & What is David Mcletchie's role as a member? & What is the result of a combination 
of a mid-life career change and a 
mid-life crisis? \\
What is about Scottish Conservative Party? & As a member, what David Mcletchie did for Scotland? & What career and family commitment made Mcletchie not put ambition into 
effect? \\
Who is David Mcletchie in Scottish Conservative Party? & Why David Mcletchie successful? & What is the result of a former leader of the Scottish Conservatives dying in a hospice in Edinburgh? \\ \bottomrule[1.5pt]

\end{tabular}
\end{center}
\caption{Different types question generation paradigms within ODQA that are related to CIS/CA. The follow-up question generation system take support of input context, responses in multiple turns provided by user, and an optional conversational planner. The information seeking type question generation is supported by passage and aims to generate a sequence of questions that makes multi-turn optional.}
\label{tab:examples_question_type}
\end{table*}

We outline the key contributions in our approach addressing the research questions defined above: 
\begin{enumerate}
    \item Knowledge-aware Passage Retriever: The component braids neural entity extraction with depth-first search-based triple extraction from the common-sense knowledge graph, ConceptNet to expand the query (Query Expander). The retriever leverage a combination of the exact entity match and soft match through maximum inner product search (MIPS) for dense retrieval of passages for question generation.
    \item Reinforcement learning-based Question Generation with Reward and Entailment Conditioned Loss: We develop a pipeline of transformers T5 and Electra working in a generative adversarial setting with a reward function of the longest common subsequence match and cosine similarity. Furthermore, we modify the model by incorporating flow in question generation by conditioning the question generation over entailment probability and reverse cross-entropy loss.
    \item We perform extensive evaluations of our proposed approach and the baseline using four evaluation metrics: (a) Rouge-L for syntactic consistency, (b) pre-trained Roberta for sentence similarity tasks for semantic relation scoring of generated and ground truth questions, (c) pre-trained Roberta for natural language inference for scoring logical agreement between generated and ground truth, (d) BERTScore  as a measure of lexical similarity, and (e) BLEURT Score for measuring grammatical consistency and semantic meaning with ground truth.
    \item Apart from the benchmarking dataset for CIS/CA, in this research, we create and present crowdsource evaluation on two real-world datasets, Depression and Anxiety, leveraging Reddit as the source of passage. Figure 2 illustrates an example from this dataset and also motivates our problem statement. 
\end{enumerate}




------------ New Dump

Open Domain Question Answering (ODQA) is seeing far reaching utility in enhancing the capabilities of conversational artificial intelligence (ConvAI) through question generation, answer retrieval, passage retrieval and passages ranking. Prior research within the sphere of information retrieval have targeted designing methods for passage retrieval and ranking given an user query. On the other hand, research within the realm of ODQA has targeted improvement in methods for question generation and answer retrieval with a limited context defined by a passage. As a consequence, the ConvAI systems have ended in being either a better reading comprehension systems or user query clarification systems that requires multi-turn follow-up question answering with the user. Further, existing ConvAI systems have shown challenges concerning the (A) context/topic drift, (B) tendency to ignore question that are semantically related and can be logically inferred from a user's query, and (C) presuming the sufficiency of the passage in question generation/answer retrieval. The (C) challenge also highlights the assumption that answer to a user query resides in one specific passage. Prior studies from \cite{zamani2020macaw}, \cite{gao2018neural}, and \cite{zhang2019addressing} have shown promising methods in addressing some of these challenges, however, the sole purpose of a user's asking a question is unaddressed, which is contextual and actionable response. Through our literature review, we found that most of the ODQA systems can benefit from the infusion of either the commonsense knowledge, domain-specific knowledge, or knowledge within the user query manifested in the form of explicit/implicit entities. 

This sense of curiosity-based question generation has far reaching benefits in healthcare 

 a novel problem of sequential information seeking type question generation (IsQG) within the ConvAI and ODQA. Essentially, IsQG system would dynamically retrieve multiple passages and generate questions t In this process we analyze the prospects of IsQG in addressing aforementioned challenges in ODQA by pairing knowledge-aware passage retriever (KPR) and neural question generator. Through IsQG, we ask the following research questions:
\begin{enumerate}
    \item Can  we  develop  a  method  that  generates a sequence  of information seeking-type questions, given an input user query? (addresses (A))
    \item Can  common-sense  knowledge  and  contextual  entities from the user’s input help in effective passage retrieving and question generation? (addresses (C))
    \item Can we generate questions that are semantically related and entailed to have a conceptual flow? (addresses (B))
    \item How do we evaluate such a method?
\end{enumerate}

To prove the feasibility and efficacy of IsQG system, we leverage conversational discourse datasets that mimics two prominent ways people seek information:  We considered four discourse datasets: (i) Conversation Assistance Track (CAsT-19) \cite{dalton2020cast}, (ii) Facebook Curiosity (FB Curiosity) \cite{rodriguez2020information}, (iii) Question Answer Discourse (QADiscourse) \cite{pyatkin2020qadiscourse}, and (iv) Question Answer Meaning Representation (QAMR) \cite{michael2018crowdsourcing}.

   Knowledge-aware   Passage   Retriever:   The   component braids  neural  entity  extraction  with  depth-first  search-based  triple  extraction  from  the  commonsense  knowledge graph, ConceptNet to expand the query. The retriever leverage a combination of the exact entity match and soft match through simple local sensitive hashing and iterative quantization (SITQ) for dense retrieval of passages for question generation.
    \item : We develop a pipeline of transformers T5 and Electra working in a generative adversarial setting with a reward function of the longest common subsequence match and cosine similarity. Furthermore, we modify the model by incorporating flow in question generation by conditioning the question generation over entailment probability and reverse cross-entropy loss.
    \item Quantitative Evaluation: We  perform  extensive  quantitative evaluations  of  RQREL for IsQG system using  five evaluation  metrics:(a)  Rouge-L  for  syntactic  consistency,  (b) RoBERTa pre-trained over semantic textual similarity for measuring semantic relatedness between generated question and ground truth, (c) RoBERTa pre-trained over stanford natural language inference for scoring logical agreement between generated question and ground truth, (d) BERTScore as a measure of lexical similarity, and (e)BLEURT Score for measuring grammatical consistency and semantic meaning with ground truth.
    \item \textcolor{red}{Qualitative Evaluation:} 
    
    The proposed novel problem definition and an approach has significant benefits for the users. Considering a social good perspective that of a mental health scenario, IsQG system can act as an information provider tool or a pre-screener and triaging tool for patients. Also, it can recommend clinicians to patient based on the conversational history. IsQG can benefit clinician by acting as a mediator in clinical interviews by providing dynamic question for information gathering. 
    
    
    \begin{table}[!htbp]
\scalebox{0.5}{
    \begin{tabular}{cp{1.6cm}p{1.6cm}p{1.6cm}p{1.6cm}p{1.6cm}p{1.6cm}}
    \toprule[1.5pt]
    \textbf{Discourse Datasets} & \textbf{Train Set} \texttt{(Avg. Qs/Iq)} & \textbf{Test Set} \texttt{(Avg. Qs/Iq)} & \textbf{Passage Source} & \textbf{\# Passages} & \textbf{\# Entities} & \textbf{\#CNetKG Triples}  \\ \midrule[1pt]
    QADiscourse  & 3131 \newline (\texttt{25})  & 825 \newline (\texttt{25})  & Wikinews + Wikipedia & 8.7Million & 96.7\% & 38.5\% \\
    
    QAMR & 24905 \newline (\texttt{63}) & 2651 \newline (\texttt{68}) & Wikinews & 3.4Million & 100\% & 35.5\% \\
    
    FB Curiosity & 50934 \newline (\texttt{6}) & 21830 \newline (\texttt{8}) & Geographic Wikipedia (Geo-Wikipedia) & 3.3Million & 100\% & 50\% \\
    
    CAST-19 & 269 \newline (\texttt{9}) & 479 \newline (\texttt{10}) & MS MARCO & 8.9 Million & 100\% & 57\% \\
    \bottomrule[1.5pt]
    \end{tabular}}
    \caption{\footnotesize Description of the datasets. \texttt{(Avg. Qs/Iq)}: Average questions per input query.}
    \label{tab:data_distribution}
\end{table}

We aim to evaluate the pipeline (KPR and RQREL) on the grounds of (a) syntactic consistency, (b) semantic consistency and conceptual flow, and (c)question legibility. Syntactic consistency in a natural language generation is defined as the capability of a generator to generate sentences that share same syntactic context as ground truth. Syntactic context relates with dependency parse tree and LCS. A higher score of LCS reflect preservation of syntactic context in generated sentence\cite{boyd2008syntactic}. We use \textbf{ROUGE-L (R-L)} score, where L stands for longest common subsequence to measure syntactic consistency. Semantic consistency measures similarity between the generated sentence and ground truth. Often models capable of generating distributed word representations are used to measure semantic consistency. We use \textbf{BERTScore} to compute lexical similarity using BERT tokenizer and model \cite{zhang2019bertscore}. Additionally, a compositional diversity can also be inferred from BERTScore and R-L score. For instance, following generated and ground truth question pair; $\hat{q}$: ``What career and family committments made Mcletchie not put ambition into effect?'' and $q$: ``What is the result of career and family commitments?'' has diverse composition causing high BERTScore and lower R-L score. 
However, BERTScore do not measure semantic relatedness between generated and ground truth sentence. To quantify semantic relations between a pair of sentences, we leverage pre-trained RoBERTa model for assessing semantic textual similarity. \textbf{Conceptual Flow (or logical agreement)} is assessed using pre-trained RoBERTa model for natural language inference \cite{kane2020nubia}. It is calculated between the generated question and ground truth. \textcolor{red}{A logical agreement score measure the}
\textbf{Question legibility} is computed using \textbf{BLEURT} score, a measure that indicate to what extent the generated question is grammatically correct and convey semantic meaning of the ground truth \cite{sellam2020bleurt}. All the metrics are specific to a task in task description and is used to compare the performance of our proposed approach with generator-only transformer-based language models.


\begin{table*}[!htbp]
\begin{tabular}{c||ccp{2.cm}p{2.cm}p{2.cm}p{2.cm}}
\toprule[1.5pt]
\backslashbox{Train}{Test} & & \textbf{Passage Source} & \textbf{QADiscourse} \newline SR/LA (\%) & \textbf{QAMR} \newline SR/LA(\%) & \textbf{FB Curiosity} \newline SR/LA(\%) & \textbf{CAST19} \newline SR/LA(\%) \\ \cmidrule{4-7}
& \textbf{Sample Size} &  & 825 & 2651 & 21830 & 479 \\ \midrule[1pt]  
QADiscourse & 3131& Wikinews + Wikipedia & \textbf{0.27/25.7} & 0.64/33.1 & 0.71/73.5 & 0.60/64.2 \\
QAMR & 24905 & Wikinews &0.28/27.7 & \textbf{0.68/37.0} & 0.75/77.8 & 0.57/58.6 \\
FB Curiosity & 50934 & Geo-Wikipedia & 0.31/33.0 & 0.67/35.8 & \textbf{0.78/79.4} & 0.67/66.5 \\
CAST-19 (50K) & 269 & MS MARCO & 0.23/25.2 & 0.61/33.4 & 0.73/76.5 & \textbf{0.61/65.0}\\ \bottomrule[1.5pt]
\end{tabular}
\caption{\textit{Semantic Relations}(SR): Assessment of M2\_RQREL in generating questions that convey the same meaning as ground truth after trained on a relatively different domain and small train sample size. \textit{Logical Agreement}(LA): measure whether the generated questions have a conceptual flow with the ground truth.}
\label{tab:domain_2}
\end{table*}


\begin{table}[t]
\scriptsize 
\begin{tabular}{p{2.cm}|p{2.cm}|p{4.cm}}
    \toprule[1.5pt]
      \multicolumn{3}{c}{\textbf{Input:} What to know about 
David Mcletchie from Scottish 
Conservative party?} \\ \midrule[1pt]
      \textbf{Clarifying Questions} & \textbf{Follow-up Questions} & \textbf{Information Seeking Questions} \\ \midrule
      (a)Who is David Mcletchie? & Who is David Mcletchie? & What is the reason he was a former 
leader of the Scottish Conservatives? \\ \midrule
 & What is David Mcletchie's role as a member? & What is the result of a combination 
of a mid-life career change and a 
mid-life crisis? \\\midrule
What is about Scottish Conservative Party? & As a member, what David Mcletchie did for Scotland? & What career and family commitment made Mcletchie not put ambition into 
effect? \\\midrule
Who is David Mcletchie in Scottish Conservative Party? & Why David Mcletchie successful? & What is the result of a former leader of the Scottish Conservatives dying in a hospice in Edinburgh? \\ \bottomrule[1.5pt]
\end{tabular}
\caption{\footnotesize Different types question generation paradigms within ODQA that are related to CIS/CA. The follow-up question generation system take support of input context, responses in multiple turns provided by user, and an optional conversational planner. The information seeking type question generation is supported by passage and aims to generate a sequence of questions that makes multi-turn optional.}
\label{tab:examples_question_type}
\end{table}



\begin{table*}[t]
\small
{\fontfamily{cmss}\selectfont
\begin{tabular}{p{5.cm}|p{5.cm}|p{6.6cm}}
    \toprule[1.5pt]
      \multicolumn{3}{c}{\textbf{Input:} What to know about David Mcletchie from Scottish Conservative party?} \\ \midrule[1pt]
      \textbf{Clarifying Questions} & \textbf{Follow-up Questions} & \textbf{Is-type Questions} \\ \midrule
      (a)Who is David Mcletchie?, (b) What is a Conservative Party?, (c)What is about Scottish Conservative Party?, (d) Who is David Mcletchie in Scottish Conservative Party? & (a) Who is David Mcletchie?, (b) What is David Mcletchie's role as a member?, (c)  As a member, what David Mcletchie did for Scotland?, (d) Why David Mcletchie successful?  & (a) What is the reason he was a former leader of the Scottish Conservatives? (b) What is the result of a combination of a mid-life career change and a mid-life crisis? (c) What career and family commitment made Mcletchie not put ambition into effect? (d) What is the result of a former leader of the Scottish Conservatives dying in a hospice in Edinburgh? \\ \bottomrule[1.5pt]
\end{tabular}}
\caption{\footnotesize Clarifying and Follow-up question generation requires multi-turn, with user giving context in each turn. Also, require a conversational planner. IsQG system involves one-shot question generation that allows the system to provide a comprehensive response without multi-turn. Also effective, if answer to query is not straightforward and requires support from multiple passages.}
\label{tab:examples_question_type}
\end{table*}



%%%%%%% 



%-----------------------

% The importance of conversation and conversational models for complex information-seeking tasks is well-established within information retrieval, initially to understand user behavior during an interactive search. However, it requires multiple turns to gather the required context to facilitate a goal-oriented dialogue addressing a user's information needs. 
% In an open domain, there is no single answer to the user query. Instead, it requires explicit knowledge to generate a sequence of questions to assist the user in gathering information. A typical information-seeking question is short and requires broad exploration of the topic by exploiting predicate and argument relationships in the sentence. Also, it spans shifting contexts across multiple passages, looks for different entity forms. Prior works in  Open Domain Question Answering (ODQA) have been in complex answer retrieval or question generation, assuming that the passage provided is relevant. An effective ODQA method is conditional upon contextual passages, and retrieving relevant passages depends on an efficient retriever.
% Further, using external knowledge through knowledge graphs, lexicons, or entity context can help retrieve relevant passages supporting legitimate question generation through curiosity. We explore a general-purpose pipeline of context-aware passage retrieval using commonsense knowledge and fine-tuning retrieval-augmented question generation for ODQA for information-seeking. For legible question generation with the conceptual flow and semantic consistency, we train the generator in a generative-adversarial setting with reinforcement learning.
% Further, we introduce an entailment loss function for generating information-seeking questions in sequence.  We extensively evaluate the proposed approach on sequential and non-sequential discourse datasets using five natural language generation metrics. Finally, we assess the working of our pipeline, end-to-end on more complex datasets: CAST-19 for conversational assistance and Real-world dataset on Depression.


%%%%% -----------

%expensive, time-consuming, and incomplete, due to lack of commonsense knowledge. We introduce a novel research problem, Information Seeking-type Question Generation (ISQG) that 
% Crowdsource discourse dataset creation -- is expensive, time-consuming, and incomplete
% 


% new abstract trying to capture the overview
% put 1 or 2 sentences to highlight information seeking need for ConvAI, first thing before saying we introduce a novel problem ,etc. -- noted


% Kalpa --- this --
%Diverse information needs of human manifested in education, healthcare, and crisis management, has attracted research in conversational artificial intelligence (ConvAI) to develop agents that support human with actionable information.  or use ``People Also Ask'' to refine the query. An appropriate response to an IS query is a compilation of small sentences from multiple passages\footnote{we say passage to consistent with the terminology in this research}.  in each turn. This can turn out to be tedious and less engaging to the human. An IS query provides minimal context, and ConvAI cannot function without an external and contextually relevant knowledge source. 

% some idea like this. Then we say we introcude our novel problem ISQG and our system to handle it called ISEEQ. I was thinking something like this. You can change or think what to do. -- noted 
% what is missing: With limited turns or possibly a single turn 
% IS query is short
%Information seeking (IS) manifested in real-world applications such as education, healthcare has attracted research in conversational artificial intelligence (ConvAI). The small size of an IS query forces ConvAI agents to perform multi-round interactions with a user to retrieve the required information. An apt response is often a compilation of small sentences from multiple passages, which the current ConvAI agents ignore. We introduce a novel research problem, Information Seeking-type Question Generation (ISQG) that enable the agent to be curious and generate multiple information seeking-type (IS-type) questions for two purposes: (i) provide human with an actionable response, and (ii) gather more information by asking in-depth questions with a limited or possibly single turn. {\fontfamily{cmss}\selectfont ISEEQ} mandates conceptual flow in question generation, and we extensively evaluate on sequential and non-sequential discourse datasets. On five natural language generation metrics, two of which introduced in this research, {\fontfamily{cmss}\selectfont ISEEQ} outperformed competitive baselines by significant margins. We assert domain adaptability of {\fontfamily{cmss}\selectfont ISEEQ} by exercising it on pairs of discourse datasets with different domains and provide a solution to ISQG.
%Therefore, enabling agent  and gather more information is inevitably important.

%However, existing conversational AI (ConvAI) agents cater to targeted information seeking needs from the users' perspective gathered through multi-round conversation and hence, lack agents' in-depth understanding of the users' requests. 

%Conversational models for complex information-seeking tasks are well-established, motivated, and supported through question answering paradigms. However, it requires multi-round interactions where the agent tries to get relevant context from the user in each turn. This can turn out to be tedious to the user. We propose an approach to automatically generate multiple information-seeking questions from single-turn short user input using external knowledge and contextually relevant data to bridge this gap. Enabling the agent to generate questions automatically helps collect user's information more efficiently and in a user-friendly manner. We generate a sequence of information-seeking questions for the short single user input query by: (i) first, retrieving semantically relevant meta-information with the help of commonsense knowledge graphs and (ii) second, training a deep generative-adversarial reinforcement learning-based question generator on both the user query and retrieved meta information to generate questions. We extensively evaluated the proposed approach on sequential and non-sequential discourse datasets using five natural language generation metrics, and it outperformed comparable baselines by significant margins.

% and in each turn tries to get user feedback as context to generate questions (or answers),. 

%%%% Introduction

% Why the targetted problem is important
%Conversational Artificial Intelligence (ConvAI) enfolds various capabilities like question generation, answer retrieval, response generation, passage retrieval, passage ranking, and others deployed within an artificial intelligence (AI) assistant to drive a meaningful and conclusive dialog with humans.  However, recent developments in ConvAI haven't progressed towards addressing the user's information needs efficiently. It is pivotal for achieving high utility of assistant during societal issues (e.g., pandemic). We believe that modeling how a user would seek information and hold dialog by asking coherent questions would help an assistant develop curiosity. Further, reducing tedious multi-turn interactions for every possible dialogue act will improve usability. Recent works on multi-turn discourse modeling or generation of question-answer hierarchies from a document attempt to seek logical coherence in conversation and plan conversational moves \cite{krishna2019generating}, \cite{li2017dailydialog}. Still, these methods can mislead the conversation in real-time as they are dependent on a single passage and drift conversation based on turn-by-turn changing user context. The presumption that answers to a user's query exist in one passage affects reflective question and response generation. In this research, we develop a novel approach to question generation within ConvAI: \textit{Information Seeking-type (Is-type) Question Generation} \textbf{(IsQG)}. 



%%%%%------ more on introduction

%Conversational Information Seeking (CIS) enfolds various capabilities like question generation, response generation, passage retrieval, passage ranking, and others to address diverse information needs of user. 

%deployed within an artificial intelligence (AI) assistant to drive a meaningful and conclusive dialog with humans. One of the main challenges in ConvAI is to keep continuous interaction with the user while addressing his information needs. However, most existing approaches in the ConvAI space try to address information-seeking behavior from the user's perspective. For example, existing assistants like Amazon Alexa and Google Assistant focus on simple question answering. They cannot gather information other than falling back to the user to provide more context in multiple rounds. In this work, we approach ConvAI from the agent's perspective to interact with the user, going beyond the purpose of finding a simple answer to the user query. We develop a novel approach to question generation within ConvAI: \textbf{I}nformation \textbf{S}eeking-type (Is-type) \textbf{Q}uestion \textbf{(ISQ)} \textbf{G}eneration \textbf{(ISQG)}.

%------------------
%Overview of our approach which illustrates IsQG system's output in two scenarios: General and Healthcare. We develop a knowledge-aware passage retriever over query expander and encoder that leverage commonsense knowledge graph. We use SITQ to retrieve top-K passages using dense representation of the query. Retrieved passages and expanded query trains generator and discriminator/evaluator in a reinforcement learning setting. Final outcome is ``p'' generated questions in ``m'' mini batches, where p defined by nucleus sampling and m is defined by number of ground-truth questions in per query in the datasets.

% To develop the IsQG system and expand the surface of ConvAI and Open Domain Question Answering (ODQA), we organize our exploration along two research questions (RQs): \textbf{(RQ1)} \textit{Knowledge-infusion}: Can expert-curated knowledge sources related to user query help in contextual passage retrieval and question generation? \textbf{(RQ2)}: Can an IsQG-based assistant generate questions that share semantic relations and logical agreement for having a conceptual flow? To address RQs, we leverage open-source discourse datasets that mimic two prominent ways Humans seek information online: (i) \textbf{\texttt{Title and Description}:} Online platforms such as Reddit showing this type of information-seeking behavior. For example: \texttt{Title:} ``I am feeling down and depressed''. \texttt{Description}: ``I am going through a rough patch in my life. With divorce proceedings and poor growth at work, I am feeling low and hopeless. What do you advise?''; (ii)\textbf{\texttt{Topic and Aspects}:} Humans seek information on Google search, Twitter, WebMD, or MedicineNet by stating topics and aspects. For example: \texttt{Topic:} ``Anxiety'' and \texttt{Aspects:} ``Panic Attacks, Trauma, Relationship, Self-detox''. For feasibility and efficacy of the IsQG system, we leverage four conversational discourse datasets, perform an evaluation with five natural language generation metrics, and conduct an unbiased human evaluation of 150 Is-type generated questions across 30 small size queries from diverse domains (e.g., history, geography, mental health, etc.).  

% research questions to answer in this work as a novel problem formulation.
% In developing a solution to the IsQG problem, we focus on solving two main research questions (RQs). They are: \textbf{(RQ1)} \textit{Knowledge-infusion}: Can expert-curated knowledge sources like knowledge graphs/bases related to user query help in context retrieval and question generation? \textbf{(RQ2)} Can an IsQG-based assistant generate questions that share semantic relations and logical coherence for having a conceptual flow? 

%To address RQs, we leverage open-source discourse datasets that mimic two prominent ways Humans seek information online: (i) \textbf{\texttt{Title and Description}:} Online platforms such as Reddit showing this type of information-seeking behavior. For example: \texttt{Title:} ``I am feeling down and depressed''. \texttt{Description}: ``I am going through a rough patch in my life. With divorce proceedings and poor growth at work, I am feeling low and hopeless. What do you advise?''; (ii)\textbf{\texttt{Topic and Aspects}:} Humans seek information on Google search, Twitter, WebMD, or MedicineNet by stating topics and aspects. For example: \texttt{Topic:} ``Anxiety'' and \texttt{Aspects:} ``Panic Attacks, Trauma, Relationship, Self-detox''. 
% For feasibility and efficacy of the ISQ system, we leverage four conversational discourse datasets, perform an evaluation with five natural language generation metrics, and conduct an unbiased human evaluation of 150 Is-type generated questions across 30 small size queries from diverse domains (e.g., history, geography, mental health, science and others). 



% Prior studies from \cite{zamani2020macaw}, \cite{gao2018neural}, and \cite{zhang2019addressing} have shown promising methods in addressing some of these challenges, however, the sole purpose of a user's asking a question is unaddressed, which is contextual and actionable response.

% We outline the key contributions of the research:
% \begin{enumerate}
%     \item \textbf{Problem:} We introduce a novel problem, IsQG within ConvAI, that would significantly improve user experience. Within IsQG, we developed a knowledge-aware pipeline of unsupervised retriever and supervised generator that would generate a sequence (or batch) of questions from a small size query that would fulfill the fine and coarse-grained information needs of a user. 
    
%     \item \textbf{Retriever and Generator:} The braided components involves semantic query expansion with explicit and implicit knowledge\footnote{explict: present in the query; implicit: present in external knowledge source}, knowledge-aware multiple passage retriever with dense query representation, and a \textbf{R}einforcement learning-based \textbf{Q}uestion Generation with \textbf{R}eward and \textbf{E}ntailment conditioned \textbf{L}oss (RQREL). 
    
%     \item \textbf{Evaluation:} We utilize RoBERTa models pre-trained on semantic textual similarity (STS) and Stanford natural language inference (SNLI) tasks for scoring logical coherence and semantic relations between generated questions and ground truth. 
    
% \end{enumerate}

% Essentially, IsQG embraces the braiding of retriever and generator guided by explicit and implicit knowledge to support the assistant in generating questions that would cover high-level topics, tailored towards fine-grained information needs of a user, and conditionally perform context switch to cover parallel by semantically related information. IsQG's sense of curiosity-based generation of questions can precisely act on the small-size user query, reduce the multi-turn, and provide a one-shot response after the user has given responses to generated questions. A detectable utility of IsQG-based assistant is in mental healthcare, in which pre-screening of user condition and its severity can help in early triaging, a challenging task for mental health practitioners (MHPs). Further, the ability to dynamically generate a question for information gathering and maintain a logical agreement between questions can make IsQG-based assistants mediate clinical interviews with MHPs. 

%%%%% more from intro
% some related work and our approach overview. Differentiate between IsQG and clarifying questions and mention we do more analytical-type complex question generation
% On the other hand, we generate more analytical and exploratory questions and, hence, can support more complex use cases. 
%Essentially, ISQG combines a context retriever and a question generator guided by explicit and implicit knowledge. Context retriever, similar to open domain QA (ODQA) systems, helps ISQG operate on open domain by generating questions based on dynamically retrieved information, and the user is given input query/question. Thus, ISQG generations are analytical and information-seeking from the agent's perspective compared to the user's perspective of asking clarifying questions. This can enable sophisticated and important real-world use cases like pre-screening and auto-triage of patients based on their current state (through short user input query - ``I am feeling dizzy'') by asking back information-seeking questions to gather more knowledge on the input query topic. To be realistic and convenient to the user, the agent tries to gather relevant knowledge from external sources and generate questions to understand the situation.


%%%%% from intro -- contributions

%We introduce a novel approach, {\fontfamily{cmss}\selectfont ISEEQ}, within CIS. We developed a knowledge-aware method by combining an unsupervised context retriever and a supervised generator. From the agent's perspective, the question generator uses the retrieved context to generate a sequence (or batch) of questions to a small size query. 

%%%% The braided components involve semantic query expansion with explicit and implicit knowledge\footnote{explicit: present in the query; implicit: present in external knowledge source}, knowledge-aware multiple context (i.e., passage) retriever with dense query representation, and a novel \textbf{R}einforcement learning-based \textbf{Q}uestion Generation with \textbf{R}eward and \textbf{E}ntailment conditioned \textbf{L}oss (RQREL) representation for this problem. 


%%%%%%% Method

%, which is a reinforcement learning-based generator-discriminator framework. The neural question generator is defined with two different optimization functions that emphasize (1) information-seeking type question set generation (Model 1: M1\_RQREL) and (2) ordered information-seeking type question generation defined by entailment probability between two generated questions (Model 2: M2\_RQREL). The reward function in both models is the same. Both the variants of RQREL consist of T5-base generator \cite{raffel2019exploring} and Electra discriminator \cite{clark2019electra}. We consider an adversarial pipeline to reward generator in creating an information-seeking question present in all the discourse datasets (Model: M1\_RQREL). Further, the pipeline also allows us to add a conditional statement to push the generator in creating questions that share semantic relations and conceptual flow (the definition of entailment in natural language inference) (Model: M2\_RQREL).In this section, we formalize the reward function and loss functions used in M1\_RQREL and M2\_RQREL.
%\\ 


%%%%%% Task Description %%%%%%%%

\texttt{T} and \texttt{D} are independently sent as input to SQE which generates intermediate outputs $E_T$ and $E_D$, a set of entities in \texttt{T} and \texttt{D} respectively (explicit knowledge). $E_T$ and $E_D$ are fed as input to triple extractor over ConceptNet, a commonsense knowledge graph (CnetKG). Output are a set of triples in the following form; $<E_T><Predicate_{R_T}><E_{O_T}>$ and $<E_D><Predicate_{R_D}><E_{O_D}>$ , where $E_{O_T}$ and $E_{O_D}$ are object entities related to head entities $E_T$ and $E_D$ (implicit knowledge). For contextualized encoding of the query with semantic information, we optimally place the triples next to the sentence having mentions of head entities $E_T$ and $E_D$. In practice, this worked better than the approach described by \cite{laugier2019encoding}. Whereas, the entities are appended to the query. Thus creating \texttt{T'} and \texttt{D'}, expanded form of \texttt{T} and \texttt{D}. 
The vector representations of \texttt{T'} and \texttt{D'} along with exact match over $E_T$ and $E_D$ is used to retrieve top-K passages ($P_{1:K}$) from the database\footnote{Wikipedia, Wikinews, and MS-MARCO passage dumps}. $P_{1:K}$ and \texttt{T'} concatenated with \texttt{D'} constitutes the context and query pairs given as input to RQREL for sequential question generation ($\hat{Q}s$). 

\noident \textbf{\texttt{Topic (Tp) and Aspects (Asp)}}: Both \texttt{Tp} and \texttt{Asp}  QE perform triple extraction over CNetKG in the similar way as in \texttt{T} and \texttt{D}. Intermediate outputs is an expanded query, \texttt{Tp'} and \texttt{Asp'} containing the entities and triple information. Following, KPR retrieves top-K passages which along with \texttt{Tp'} and \texttt{Asp'} generate a sequence of $\hat{Q}s$.  Such an input query defines a case where the user provides clues describing their information needs without details. 
% \item \texttt{Description (D) only}: This variant differs from \texttt{T and D} and \texttt{Tp and Asp} as it provide a complex descriptions with many $E_D$ which may or may not be related to each others. QE does initiate the entity extractor and triple extractor but the chances of strong hit in CNetKG is low. With a focus to develop a generalizable pipeline for CIS/CA, we pass $E_D$ and triples to KPR for $P_{1:K}$ retrieval. The modified description (\texttt{D'}) and $P_{1:K}$ are used to generate a sequence of $\hat{Q}s$.  


%%%%%%%% from Approach





\textcolor{red}{Further, extracted entities are appended to \texttt{D'} forming the output for KPR.}



 



 For instance, $E_T$ and $E_D$ are identifiable noun phrases or verb phrases\footnote{a noun/verb phrase, if exist in a KG, is called an entity} in \texttt{\textbf{T and D}} used to gather triples from CnetKG in the following form:  $<E_T><Predicate_{R_T}><E_{O_T}>$ and $<E_D><Predicate_{R_D}><E_{O_D}>$ , where $E_{O_T}$ and $E_{O_D}$ are object entities related to head entities $E_T$ and $E_D$. We insert the triples next to the sentence mentioning head entities $E_T$ and $E_D$. And later append $E_T$ and $E_D$ to query. From here, we term the semantically expanded query as \textit{kquery}. In practice, this worked better than the approach described by \cite{laugier2019encoding}.  Second, \textit{kquery} yields context-rich encoding using any language model and facilitates retrieval of passages that are to the point. It is conducted by a knowledge-aware passage retriever, which also ranks the passages. Further, re-ranking is performed by checking the presence/absence of $E_T$ and $E_D$ in retrieved passages. Third, retrieved passages and \textit{kquery} is used by neural question generator to generate IS-type questions. 
 



is performed in three steps: (a) Entity Extraction, (b) Multi-hop triple extraction from knowledge graph, and (c) Query expansion. 



 or $E_T$ or \texttt{Tp} or \texttt{Asp}. 
A  retrieved and 

or $E_T$ or \texttt{Tp} or \texttt{Asp}. 

% \mbox{SITQ} \equiv Pr_{\mbox{top-K}}(passages|\vec{\mathbb{P}},\vec{kq})
\noindent 

Similar process can be followed for other types of IS queries. 



 %%%%%%%% KPR
\paragraph{KPR:} It is made with specific improvements over \cite{lewis2020retrieval}: (a) method for encoding passages and query, (b) algorithm for passage retrieval, and (c) heuristics for passage filtering. Input to KPR is the expanded query from SQE and an index of passages ($\mathbb{P}$). Dense encoding of a passage ($\mathbf{P}(\textit{z}$) $\in \mathbb{P}(\mathcal{Z})$)  and query ($\mathbf{q}(x) \in \texttt{T'and D'} or \texttt{Tp'and Asp'}, or \texttt{D'}$) is created using Sentence-BERT (S-BERT) \cite{reimers2019sentence}. It can be defined as: 
\begin{align}
\mathbf{P}(\textit{z}) = \mbox{S-BERT}_{P}(\textit{z});
\mathbf{q}(x) = \mbox{S-BERT}_{q}(\textit{x}); \\
Pr_{\mbox{top-N}}(P|q) \propto \mbox{top-N} \{{exp(\mathbf{q}(x)^T\mathbf{P}(\textit{z}))}_{\mathbf{P} \in \mathbb{P}}\}
\end{align}
KPR uses SITQ (Simple local sensitive hashing (Simple-LSH) and Iterative Quantization), an algorithm for fast maximum inner product search (MIPS) to retrieve a rank list of passages from the indexed database.  SITQ ($Pr_{\mbox{top-N}}(P|q)$) converts dense representations into low-rank vectors and learns transformation matrix between input query and passage \cite{khattab2020colbert} \cite{neyshabur2015symmetric}. Passages are ranked by similarity, a soft match retrieval. Further, after top-N passages are retrieved ($\mathbf{P}_{1:N}$), we re-rank by a normalized entity score, calculated for each $P_i \in \mathbf{P}_{1:N}$ as $\frac{\sum_{e_j \in E_D'} \{\mathbb{I}(e_j = w)\}_{w \in P_i}}{|E_D'|}$ and arrange in descending order. We kept those top-K passages ($\mathbf{P}_{1:K}$) with normalized entity score\footnote{an entity occurring multiple times in $P_i$ will be counted once} $>$80\%. This heuristic worked well as it covers all the major entities in \texttt{D'}. We tested the efficiency of KPR with comparable baselines on the QAMR Wikinews dataset \footnote{wikinews are complex because of sudden changes in context. An article on Liam Aitchson Murder Case contains information on attention deficit hyperactivity disorder and other murder cases in Scotland}. Table \ref{tab:retriever} shows performance improvements of KPR and its variants (KPR-E: \texttt{D'} has only entities and KPR-ET: \texttt{D'} has entities and triples). Mean Average Precision (MAP) is calculated with respect to ground truth questions in QAMR. There are two components in MAP:(a) \textit{Relevance} of the retrieved passage in generating questions that have $>$70\% cosine similarity with ground truth; (b) Normalize \textit{Relevance} by the number of ground truth questions per input query. To get MAP, we multiple (a) and (b) and take mean over all the input queries. We do MAP calculation over top-20 retrieved passages because of the good confidence in hit rate.


%%%%%%%%%% From approach -- reward function and all

\paragraph{{\fontfamily{cmss}\selectfont ISEEQ-RL} and {\fontfamily{cmss}\selectfont ISEEQ-ERL}:}
%\todo[inline]{Model 1 and Model 2}
The retrieved passages ($\mathbf{P}_{1:K}$) and the modified input queries (\texttt{T'and D'} or \texttt{Tp'and Asp'}) fine tune paired transformers in a generative-adversarial framework using reinforcement learning for IS-type QG. The pairing includes a T5-base generator \cite{raffel2019exploring} and Electra discriminator \cite{clark2019electra} that leverage a reward function to balance two capabilities: (a) generate question having overlap with ground truth, and (b) generate question that is compositional diverse but semantically similar to ground truth. Subsequently, we elaborate on the reward function and formalize the optimization and learning in {\fontfamily{cmss}\selectfont ISEEQ-RL} and {\fontfamily{cmss}\selectfont ISEEQ-ERL}. 




\begin{equation}
\label{eq:1}
    \alpha\bigg[\frac{LCS(\hat{q}_{i}^{n},q_{i}^{n})}{|\hat{q}_{i}^{n}|}\bigg]+(1-\alpha)\bigg[\sum_{\hat{w_{ij}}\in\hat{q}_{i}^{n}}\max_{w_{ik}\in q_{i}^{n}}(\hat{w_{ij}}^{T}w_{ik})\bigg]
\end{equation}

where $\bigg[\frac{LCS(\hat{q}_{i}^{n},q_{i}^{n})}{|\hat{q}_{i}^{n}|}\bigg]$ is a measure of longest common subsequence (LCS) overlap between $q^n_i$ and $\hat{q}^n_i$. This part of the equation \ref{eq:1} capture word order, explicit information through exact match and restricts the generator from generating non-information seeking questions. Other part of the equation \ref{eq:1} allows for a soft measure of similarity instead of exact match. We leverage tokenizer provided with BERT to tokenize $q^n_i$ and $\hat{q}^n_i$, the embedding model generate a sequence of vectors, one for each tokens. Soft match is required in the reward to account for semantic similarity and compositional diversity. For instance, to generate the following information-seeking question: $\hat{q}^n_i$=``What is the average earnings of nurse in UK?" for a $q^n_i$ = ``What is the average starting salary in the UK?", soft match is required in $R_i$. The hyperparameter $\alpha$ balance the soft match with exact match.


%%%%%%%%% ISEEQ-ERL

\noindent \textbf{Cross Entropy (CE) Loss in {\fontfamily{cmss}\selectfont ISEEQ-RL}:} Since the queries in the discourse datasets varies in context, we compute CE loss in batches and tune the CE loss, calculated over all input queries after each epoch.
We end-to-end train a generator and discriminator in mini-batches of $q^n_i$ and $\hat{q}^n_i$ with batch-size ``m'', defined by the number of $q^n_i$s for an input query. The loss in {\fontfamily{cmss}\selectfont ISEEQ-RL} is defined as:
\begin{equation}
\label{eq:2}
    \mathcal{L}(\hat{q}_{1:m}|q_{1:m},\theta) = \frac{-\sum_{i=1}^m R_i\cdot\mathbb{I}(q^n_i=\hat{q}^n_i)\cdot\mathbf{log}Pr(\hat{q}^n_i)}{m}
\end{equation}
where $\mathbb{I}(q^n_i=\hat{q}^n_i)$ is an indicator function that returns the match of word indices between $q^n_i$ and $\hat{q}^n_i$. The CE loss over all the input queries in a discourse dataset is $\mathcal{L}(\hat{Q}|Q,\Theta)$, which is recorded after an epoch ``t''. The tuning of $\mathcal{L}(\hat{Q}|Q,\Theta)$ is defined as:
\begin{equation}
\label{eq:3}
\mathcal{L}(\hat{Q}|Q,\Theta)_t = \gamma \mathcal{L}(\hat{Q}|Q,\Theta)_{t-1} + (1-\gamma)\mathcal{L}(\hat{q}_{1:m}|q_{1:m},\theta)
\end{equation}
Equations \ref{eq:1} and \ref{eq:2} are responsible for generating information-seeking questions the are appropriate to input query concerning the context and can semantically paraphrase the question based on the triples and entity information in the input query. 
Since {\fontfamily{cmss}\selectfont ISEEQ-RL} is exposed to input query and retrieved passages, answers are present for the generated information-seeking questions. We show the improvement in the performance of {\fontfamily{cmss}\selectfont ISEEQ-RL} by conducting an ablation study over input query, passages, entities, and triples. 

\noindent \textbf{Entailment with Reverse Cross-Entropy loss in {\fontfamily{cmss}\selectfont ISEEQ-ERL}:} Information gathering questions should be semantically related and coherent with user query to prevent off-tracking IS task in CIS. For instance, given an input query of the form: \texttt{D:} Bothered by feeling down, depression, and hopelessness. The generated questions from the {\fontfamily{cmss}\selectfont ISEEQ-RL} are: ($\hat{q}_a$) What is the reason for the depression, hopelessness? ($\hat{q}_b$) What is the frequency of you feeling down and depressed? Whereas, {\fontfamily{cmss}\selectfont ISEEQ-ERL} would place ($\hat{q}_b$) question before ($\hat{q}_a$) as the entailment probability of ($\hat{q}_b$) given ($\hat{q}_a$) is smaller than ($\hat{q}_a$) given ($\hat{q}_b$). We condition equation \ref{eq:2} over an entailment label provided by a RoBERTa model, pre-trained on ``Stanford natural language inference (SNLI)'' task \cite{tarunesh2021trusting}. For defining the loss function in {\fontfamily{cmss}\selectfont ISEEQ-ERL}, we consider  $\hat{q}^n_{i|entail}$, a question in the list of generated questions (in a mini-batch) having $n$ tokens and is a successor to $\hat{q}^n_{i}$.
We calculate the entailment probability as:

\[
\mbox{label}(\hat{q}^n_i, \hat{q}^n_{i|entail}) = \mbox{arg}\max \mbox{RoBERTa}(\hat{q}^n_i, \hat{q}^n_j)\]
\[
\mbox{label}(\hat{q}^n_i, \hat{q}^n_{i|entail}) \in \mbox{\{neutral, contradiction, entailment\}}
\]
\[
Pr(\hat{q}^n_i, \hat{q}^n_{i|entail}) = \max\mbox{RoBERTa}(\hat{q}^n_i, \hat{q}^n_j)
\]

\begin{algorithmic}
\label{eq:4}
  \IF{$\mbox{label}(\hat{q}^n_i, \hat{q}^n_{i|entail}) = \mbox{entailment}$}
    \STATE  $\mathcal{L}(\hat{q}_{1:m}|q_{1:m},\theta)=$
    \STATE  $ - \bigg(\frac{\sum_{i=1}^m R_i \cdot \mathbb{I}(q_i=\hat{q}_i) \cdot \mathbf{log}Pr(\hat{q}_i)}{m} + Pr(\hat{q}^n_i, \hat{q}^n_{i|entail})\bigg)$
  \ELSE
    \STATE $\mathcal{L}(\hat{q}_{1:m}|q_{1:m},\theta) =$ 
    \STATE $-\bigg(\frac{\sum_{i=1}^m R_i(1-\mathbb{I}(q_i=\hat{q}_i))Pr(\hat{q}_i)}{m} +(1-Pr(\hat{q}^n_i, \hat{q}^n_{i|entail}))\bigg)$
  \ENDIF
\end{algorithmic}

where $-\bigg(\frac{\sum_{i=1}^m R_i(1-\mathbb{I}(q_i=\hat{q}_i))Pr(\hat{q}_i)}{m}\bigg)$ is termed as reverse cross-entropy (RCE). In {\fontfamily{cmss}\selectfont ISEEQ-ERL}, we want to discourage the generation of non-entailed questions by minimizing the sum of RCE and complement of entailment probability.  Any further improvement to {\fontfamily{cmss}\selectfont ISEEQ-ERL} is left to future work.


%%%%%%%%% evaluation

We evaluate {\fontfamily{cmss}\selectfont ISEEQ} generations using Rouge-L (R-L), BERTScore (BScore) \cite{zhang2019bertscore}, and BLEURT (BRT) \cite{sellam2020bleurt} that respectively measures preservation of syntactic context, semantics, and legibility of question to human understanding. For conceptual flow in question generation, we define ``semantic relations'' (SR) and ``logical coherence'' (LC) metrics. To quantify SR between a pair of sentences, we leverage the pre-trained RoBERTa model for assessing semantic textual similarity. LC is calculated by counting the number of entailment labels between pair of ground truth and generated questions. LC is reported in percentage by summing the count and dividing by the $|\hat{Q}|$ across $\mathbf{K_D}$ in a discourse dataset.   

\footnote{https://huggingface.co/textattack/roberta-base-STS-B}. LC is assessed using the pre-trained RoBERTa model for SNLI\footnote{https://paperswithcode.com/lib/allennlp/roberta-snli}


%%%%%%%%%%%%%%%% Results ISEEQ-RL ISEEQ-ERL

%7.5\% improvement in R-L in QAMR dataset  
%13\% improvement in BRT, 7\% BScore, 6\% SR, 30\% LC in QAMR dataset
%2-15\% improvement from RL to ERL in QAMR 

%3\% in BRT, 4\% in SR, 5\% in LC in FBC
%6\% in RL 2.2 in BRT, 5\% in BScore, 6\% in SR, 10\% in LC in FBC 

%Properties within ISEEQ
%1. What does semantic expansion of the query brings in:
%2. What benefit you achieve by having multiple passages:
%3. you are getting questions in one shot 
\paragraph{Performance of {\fontfamily{cmss}\selectfont ISEEQ-RL} and {\fontfamily{cmss}\selectfont ISEEQ-ERL} :} Datasets used in this research were designed for a CIS agent to obtain the capability of multiple contextual passage retrieval and one-shot diverse IS-type QG. The process of creating such datasets require crowd workers take the role of CIS agents for question creation and evaluators to see whether questions match the information needs in the query. Implicitly, the process embeds crowd workers' curiosity-driven search to read multiple passages for IS-type question creation. Baselines employed in developing CIS agent works on single passage-based QG with much of the efforts focusing on improving QG. Whereas {\fontfamily{cmss}\selectfont ISEEQ} generation enjoys the success from the connection of SQE, KPR, and novel QG model over baselines in CIS (see Table \ref{tab:major_results}). With SQE, {\fontfamily{cmss}\selectfont ISEEQ} achieved \mbox{2-6\%} across all discourse datasets.
The knowledge-infusion in {\fontfamily{cmss}\selectfont ISEEQ} through SQE has shown to be powerful for baselines as well. Table \ref{tab:major_results} records \mbox{3-10\%, 3-10\%, and 1-3\%} performance gains of the baselines on QAD, QAMR, and FBC across five evaluation metrics, respectively. SQE allows baselines to semantically widen their search over the gold passages in datasets to generate diverse questions that match better with ground truth. Differently, {\fontfamily{cmss}\selectfont ISEEQ-RL} generations benefit from dynamic meta-information retrieval from multiple passages yielding hike of \mbox{20-35\%, 6-13\%, 3-10\%} on QAD, QAMR, and FBC, respectively, across five evaluation metrics. Especially, QG in CAsT-19 and FBC dataset advance because of KPR in  {\fontfamily{cmss}\selectfont ISEEQ-RL} and {\fontfamily{cmss}\selectfont ISEEQ-ERL} (see Figure \ref{fig:cast19_results}). Most of the CAsT-19 and FB Curiosity (FBC) queries required multiple passages to construct legible questions. For instance, Is-type question: ``Enquiry about History, Economy, and Sports in Hyderabad'' requires three passages on ``History\_Hyderabad'', ``Economy\_Hyderabad'', and ``Sports\_Hyderabad'' which were missing in gold passages. Thus, TLM-FT baselines find it hard to construct legible IS-type questions using the gold passage. Furthermore, {\fontfamily{cmss}\selectfont ISEEQ-ERL} advance the quality of QG over {\fontfamily{cmss}\selectfont ISEEQ-RL} by 7-14\% and 6-10\% in QAD and FBC.  QAD and FBC questions require QG model to emphasize on conceptual flow.

%3\% 6\% 10\% 7\% 14\%-- QAD
%7\% 6\% 8\% 4\% 6\%  -- QAMR
%6\% 2\% 5\% 6\% 10\% -- FBC

----------------------------------------------

Table \ref{tab:major_results} shows that infusion of knowledge in queries significantly improves natural language question generation in open domain. Particularly in  T5-FT CANARD, which stood out as the most competitive baseline. It is because of the question-in-context rewriting capability that focuses on syntactic and semantic consistency. However, it is not aware of semantic relations and logical coherence in question generation. Thus, {\fontfamily{cmss}\selectfont ISEEQ-ERL} significantly outperformed T5-FT CANARD and other baselines by large margins across all the five metrics. Even {\fontfamily{cmss}\selectfont ISEEQ-RL} without SQE equals T5-FT CANARD. Furthermore, it shows that retrieval of multiple relevant passages by KPR surpassed single passage TLMs, often considered in prior works in CIS. 


 {\fontfamily{cmss}\selectfont ISEEQ-RL} and {\fontfamily{cmss}\selectfont ISEEQ-ERL} prevented the loss by finding answers in passages that share semantic relations to gold passages. It showed that models generated legible questions that have semantic relations and logical coherence with ground truth. Ablations on encodings were performed to experiment separate contributions of KPR ($\mathbf{P}_{1:K}$) and SQE in question generation. Table \ref{tab:ablation} records an average improvement of 2-6\% across all discourse datasets.
 
 
 %%%%%%%%% CAST-19 
 
 -------------------------

 CAsT-19 presents a unique real-world challenge in terms of diverse context and semantic phenomena on a small dataset. Experiments on CAsT-19 assessed the combined utility of KPR and {\fontfamily{cmss}\selectfont ISEEQ-ERL}. For each input query, in any iteration of KPR, top-100 passages were retrieved and checked for the presence of $>$80\% of the entities (exact match). KPR is stopped after each query in the train set has at least one passage. With $\sim$50K passages KPR fulfilled to task compared to DPR. Further, KPR-E and KPR-ET retrieved passages for 75\% and 84\% of input queries in the CAsT-19 test, respectively. Whereas DPR support 30\% queries in train set (see Table \ref{tab:cast19_1}). Figure \ref{fig:cast19_results} (a) illustrates the quality of {\fontfamily{cmss}\selectfont ISEEQ-RL} generations on the CAsT-19 dataset, which are 27\% more semantic similar and related with the ground truth compared to T5-FT CANARD. {\fontfamily{cmss}\selectfont ISEEQ-RL} with SQE generated 54\% questions that entail a ground truth question in CAsT-19\footnote{it means of 10 generated questions, 5 or 6 can be logically inferred from ground truth question} (Figure \ref{fig:cast19_results}(b).(KPR-E)+{\fontfamily{cmss}\selectfont ISEEQ-ERL} and (KPR)-ET+{\fontfamily{cmss}\selectfont ISEEQ-ERL} seems to generate Is-type questions with significantly large logical coherence and concept flow. Moreover, figure \ref{fig:cast19_results}(c,d) illustrates the remarkable improvement in the generation of questions with the conceptual flow with a lower number of retrieved passages on a highly complex CAsT-19 dataset. We attribute this to the addition of loss function optimizers: entailment probability and RCE.
 
 
 %%%%%% Figure 3 caption
 
 
 \footnotesize (a) and (b): Generation scores of the pipeline: KPR combined with {\fontfamily{cmss}\selectfont ISEEQ-RL} and {\fontfamily{cmss}\selectfont ISEEQ-ERL} on CAsT-19 Dataset. (c) and (d): Substantial improvement in generations because of entailment loss in {\fontfamily{cmss}\selectfont ISEEQ-ERL}. Baseline: T5-FT CANARD.
 
 
 \multirow{3}{*}{ProphetNet-FT SQUAD} &-& 0.24 & 0.38 & 0.11 & 0.17 & 11.0 & 0.23 & 0.61 & 0.39 & 0.37 & 17.7 
& 0.56 & 0.68 & 0.51 & 0.60 & 57.3 \\
& +\textcolor{OliveGreen}{Entities} & 0.26 & 0.39 & 0.13 & 0.17 & 11.0 & 0.29 & 0.62 & 0.41 & 0.37 & 18.1 
& 0.58 & 0.70 & 0.51 & 0.62 & 58.4 \\
& +\textcolor{blue}{Triples} & 0.27 & 0.41 & 0.17 & 0.17 & 11.0 & 0.34 & 0.65 & 0.43 & 0.38 & 19.0 
& 0.58 & 0.72 & 0.50 & 0.63 & 59.7 \\ \cmidrule{2-17}


%%%%%%%%%%% Domain Adaptation %%%%%%%%%%%%%%

Experiments with {\fontfamily{cmss}\selectfont ISEEQ-ERL} on discourse datasets from diverse domains establish it as a promising model for CIS. Also, it posits RQ3, an answer to which would illuminate the potential of {\fontfamily{cmss}\selectfont ISEEQ-ERL} in creating other datasets involving minimal to no crowd workers. Table \ref{tab:domain_1} shows training of {\fontfamily{cmss}\selectfont ISEEQ-ERL} on FBC yield far better results on QAD, QAMR, and CAsT-19 than in-domain train and test of {\fontfamily{cmss}\selectfont ISEEQ-ERL}. Regardless of the large train size of FBC, it is narrow in domain compared to other datasets. Cross-domain test results on QAD, QAMR, and CAsT-19 provide a compelling position on {\fontfamily{cmss}\selectfont ISEEQ-ERL}'s ability to create new datasets for CIS agent training and development. Table \ref{tab:domain_1} shows other successful cross-domain results in blue boxes\footnote{we tested overlap between retrieved passages in QAD, QAMR, FBC, and CAsT-19. They showed statistical difference with p-value<0.05.}.



------------------------------------
\paragraph{Domain Adaptation:} {\fontfamily{cmss}\selectfont ISEEQ-ERL} is trained and tested on datasets covering different domains. For instance, training on QADiscourse, which covers articles from WikiNews, and testing on CAsT-19 covering articles from the web (science, health, history, etc.). Performance scores on five metrics examine the generalizability of {\fontfamily{cmss}\selectfont ISEEQ-ERL}. Table \ref{tab:domain_1} records improvement in IsQG in CAsT-19 by 2\% on R-L, 6\% on BScore, 2\% on SR, and 1.2\% on LC after M2\_RQREL was trained on QAD. Further, training {\fontfamily{cmss}\selectfont ISEEQ-ERL} on QAMR presented results on the FBC test set comparable to the experiment involving train-test on FBC. Likewise, training {\fontfamily{cmss}\selectfont ISEEQ-ERL} on QAD and testing on QAMR presented results which are close to train-test on QAMR\footnote{we tested overlap between retrieved passages in QAD, QAMR, FBC, and CAsT-19. They showed statistical difference with p-value<0.02}.



%%%%%%%%%%% Human Evaluation 

--------------------------------------
 We carried out 12 blind evaluations. Evaluators did not know which system is ground truth (S1), {\fontfamily{cmss}\selectfont ISEEQ-ERL}(S2), and T5-FT CANARD (S3) \footnote{All the evaluators were allowed to use web resources for side information on queries to perform high-quality assessments}. Evaluators rate ISQs along five guidelines (G) created using qualitative studies in CIS\cite{schank1977rules}\cite{lehnert1977process}:
G1: Are the questions in a well-formed English language; G2: Are the questions rich in gathering relevant context?; G3: Are the questions diverse and non-redundant?; G4 Are the question logically coherent?; and G5: Which system would they pick for addressing their information needs? Each of these questions got integer scores between 1 (low) to 5 (high). Each human evaluation comprises 30 user queries covering domains such as Health, Science, History, Geography. On average, S1, S2, and S3 generated 7, 7, 5 ISQs per query, respectively, generating . We examined the ratings of systems on G1-G5 for variance using one-way ANOVA. If a pair of systems, for instance, S1\&S2, receive ratings on G1 with no significant variance, we consider these systems to be similar in performance on G1. On the other hand, if there is a statistically significant difference, we perform a one-tailed Wilcoxon signed-rank test to see which system gained confidence in evaluators. From Table \ref{tab:human_eval}, we make following interpretations: \textbf{(1)} For G1, there was a significant variance in ratings between S2\&S3, with evaluators' findings S2 generated questions to be more legible than S3. However, S1\&S2 and S1\&S3 had ratings with marginal variations. \textbf{(2)} G2, G3, and G4 evaluations suggested S2 effectively contextual information gathering over S1 and S3. This also addresses \textbf{RQ2} that emphasizes logical coherence and semantic relations for efficient CIS. \textbf{(3)} G5 mainly ask evaluators, 


``Which system would they pick for addressing their information needs?'' and we found them selecting S1 and S2 in the majority. However, based on our feedback, for a few complex queries, such as ``Need help. Bothered by little interest or pleasure in doing things'', ``Need to know about Gemini VIII. Armstrong used an emergency set of thrusters to regain control. Gemini VIII landed in the Pacific Ocean after ten hours of flight''; they were indecisive between S2 and S3, giving them the same ratings (wp=0.09 $<$ 0.1).

%%%%%%%%%% Modified Human Evaluation %%%%%%%

\paragraph{Human Evaluation:} We carried out 12 blind evaluations of 30 information seeking queries covering Health, Science, History, and Geography. Each evaluator rate (scores between 1 (low) to 5 (high)) 570 ISQs (6,240 ratings) according to five guidelines (G) for assessing CIS \cite{schank1977rules}\cite{lehnert1977process}:G1: Are the questions in a well-formed English language; G2: Are the questions rich in gathering relevant context?; G3: Are the questions diverse and non-redundant?; G4 Are the question logically coherent?; and G5: Which system would they pick for addressing their information needs?. For each G, we perform one-way ANOVA to check statistically significant variance (p-value$<$0.1, Table \ref{tab:human_eval}) in systems' ratings. Further, per G, Wilcoxon signed rank test was performed over a pair of systems with p-value$<$0.1 on one-way ANOVA. From Table \ref{tab:human_eval}, we make following interpretations per G: \textbf{(G1):} Evaluators found S1, S2, and S3 to be capable of generating legible ISQs.\textbf{(G2 and G3):} Across 30 queries, evaluators found S1 and S2 generating ISQs that are relevant, cover diverse context of input query and non-redundant\footnote{some evaluators took web help to affirm their ratings} compare to S3. \textbf{(G4 and G5):} {\fontfamily{cmss}\selectfont ISEEQ-ERL}'s generated ISQs that match the quality of crowd workers employed in creating QAD, QAMR, FBC, and CAsT-19 (addresses RQ3). For some queries, {\fontfamily{cmss}\selectfont ISEEQ-ERL}' generations showed better conceptual flow than ground truth (wp value are close to significance levels in table \ref{tab:human_eval}).


\begin{table}[!ht]
\scalebox{0.9}{
{\fontfamily{cmss}\selectfont
\begin{tabular}{p{0.5cm}p{2.4cm}p{2.4cm}p{2.4cm}}
\toprule[1.5pt]
&  \textbf{S1\&S2} & \textbf{S1\&S3}  & \textbf{S2\&S3} \\ \midrule[1pt]
G1 & S1$==$S2^{$\mathsection$} & S1==S3^$\mathsection$ & S2==S3^$\mathsection$ \\
G2 & S1==S2^$\mathsection$	& S1$>$S3^$\dagger$ (wp=0.003) & S2$>$S3^$\dagger$ (wp=0.005) \\
G3 & S2==S1^$\mathsection$ & S1$>$S3^$\dagger$ (wp=1.00E-04) & S2$>$S3^$\dagger$ (wp=2.18E-05) \\
G4 & S2$>$S1^$\dagger$ (wp=0.0034) & S1$>$S3^$\dagger$ (wp=0.0012)	& S2$>$S3^$\dagger$ (wp=2.03E-10) \\
G5 & S2$>$S1^$\dagger$ (wp=0.042) & S1==S3^$\mathsection$ & S2$>$S3^$\dagger$ (wp=0.015) \\
\bottomrule[1.5pt]
\end{tabular}}}
\caption{\footnotesize Assessment of human judgements on crowd worker's ISQs, ISEEQ-ERL, and T5-FT CANARD. 
$\mathsection$: ANOVA p-value$>$0.05, $\dagger$: ANOVA p-value$<$0.05 and Wilcoxon p-value (wp)$<$0.05. Note: Ratings of S1\&S3 with respect to G5  was not significant at 0.05 (p=0.069) but significant at p$<$0.1. $\mathbf{==}$: systems' ratings are same and $\mathbf{>}$: systems ratings are different and one system is better than other.}
\label{tab:human_eval}
\end{table}




\pgfplotstableread[col sep=comma,]{data.csv}\datatable


\pgfplotsset{colormap/violet}\pgfplotstableread[col sep=comma,]{data2.csv}\datatables


\pgfplotstableread[col sep=comma,]{data3.csv}\datatabless


\pgfplotstableread[col sep=comma,]{data4.csv}\datatablesss



\vspace{-1em}
%--------------------------------
\begin{minipage}[h]{1.0\linewidth}
\centering
\subfloat[][]{\resizebox{0.5\textwidth}{!}{
\begin{tikzpicture}
\begin{axis}[legend style={nodes={scale=0.6, transform shape}}, width=7.5cm, height=5.5cm,
    ybar,
    bar width=5pt,
    xlabel={Retrieved Passages},
    ylabel={Semantic Relations},
    xtick=data,
    xticklabels from table={\datatabless}{A},
    ymajorgrids,
    legend pos=north west
             ]
    \addplot table [x expr=\coordindex, y= B]{\datatabless};
    \addplot table [x expr=\coordindex, y= C]{\datatabless};
    \addplot table [x expr=\coordindex, y= D]{\datatabless};
    \addplot table [x expr=\coordindex, y= E]{\datatabless};
    \legend{KPR($z_{E_D}$)+{\fontfamily{cmss}\selectfont ISEEQ-RL},KPR($z_{E_D}$)+{\fontfamily{cmss}\selectfont ISEEQ-ERL},KPR($z_{K_D}$)+{\fontfamily{cmss}\selectfont ISEEQ-RL}, KPR($z_{K_D}$)+{\fontfamily{cmss}\selectfont ISEEQ-ERL}}
\end{axis}
\end{tikzpicture}}}
\subfloat[][]{\resizebox{0.5\textwidth}{!}{
\begin{tikzpicture}
\begin{axis}[legend style={nodes={scale=0.6, transform shape}}, width=7.5cm, height=5.5cm,
    ybar,
    bar width=5pt,
    xlabel={Retrieved Passages},
    ylabel={Logical Coherence},
    xtick=data,
    xticklabels from table={\datatablesss}{A},
    ymajorgrids,
    legend pos=north west
             ]
    \addplot table [x expr=\coordindex, y= B]{\datatablesss};
    \addplot table [x expr=\coordindex, y= C]{\datatablesss};
    \addplot table [x expr=\coordindex, y= D]{\datatablesss};
    \addplot table [x expr=\coordindex, y= E]{\datatablesss};
    \legend{KPR($z_{E_D}$)+{\fontfamily{cmss}\selectfont ISEEQ-RL},KPR($z_{E_D}$)+{\fontfamily{cmss}\selectfont ISEEQ-ERL},KPR($z_{K_D}$)+{\fontfamily{cmss}\selectfont ISEEQ-RL}, KPR($z_{K_D}$)+{\fontfamily{cmss}\selectfont ISEEQ-ERL}}
\end{axis}
\end{tikzpicture}}}
\end{minipage}



\begin{figure}[!ht]
{\fontfamily{cmss}\selectfont
\begin{minipage}[h]{0.5\linewidth}
\centering

\begin{tikzpicture}
\begin{axis}[legend style={nodes={scale=0.45, transform shape}}, width=9.cm, height=4.cm,
    ybar,
    bar width=5pt,
    xlabel={Retrieved Passages},
    ylabel={SR},
    xtick=data,
    xticklabels from table={\datatable}{A},
    ymajorgrids,
    legend pos=north west,
    legend image code/.code={%
                    \draw[#1, draw=none] (0cm,-0.1cm) rectangle (0.6cm,0.1cm);
                }
             ]
    \addplot table [x expr=\coordindex, y= B]{\datatable};
    \addplot table [x expr=\coordindex, y= C]{\datatable};
    \addplot table [x expr=\coordindex, y= D]{\datatable};
    \legend{Baseline, KPR($\mathcal{Z}_{k_d}$)+{\fontfamily{cmss}\selectfont ISEEQ-RL}, KPR($\mathcal{Z}_{k_d}$)+{\fontfamily{cmss}\selectfont ISEEQ-ERL}}
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[legend style={nodes={scale=0.45, transform shape}}, width=9.cm, height=4.cm,
    ybar,
    bar width=5pt,
    xlabel={Retrieved Passages},
    ylabel={LC(\%)},
    xtick=data,
    xticklabels from table={\datatables}{A},
    ymajorgrids,
    legend pos=north west,
    legend image code/.code={%
                    \draw[#1, draw=none] (0cm,-0.1cm) rectangle (0.6cm,0.1cm);
                }
             ]
    \addplot table [x expr=\coordindex, y= B]{\datatables};
    \addplot table [x expr=\coordindex, y= C]{\datatables};
    \addplot table [x expr=\coordindex, y= D]{\datatables};
    \legend{Baseline, KPR($\mathcal{Z}_{k_d}$)+{\fontfamily{cmss}\selectfont ISEEQ-RL}, KPR($\mathcal{Z}_{k_d}$)+{\fontfamily{cmss}\selectfont ISEEQ-ERL}}
\end{axis}
\end{tikzpicture}
\end{minipage}}




% As mentioned earlier, $k_d$ is used as the input to the passage retriever, resulting in top-K passages. We denote a passage as $p$ and the set of passages as $\mathbf{P}$. Thus, we denote the top-K passages retrieved as ($\mathbf{P}_{\mbox{top-K}}$).

% We made specific improvements over the Dense Passage Retriever (DPR) described in \cite{lewis2020retrieval}: (a) encoder for the passages $p \in \mathbf{P}$ and $k_d$, and (b) algorithm for top-K passage retrieval ($\mathbf{P}_{\mbox{top-K}}$) %\todo[inline]{do you mean to say N or K??} 
% by using a normalized entity score (NES) to pick $\mathbf{P}_{\mbox{top-K}}$. We create dense encodings of $p \in \mathbf{P}$ using Sentence-BERT, which is represented as $\mathcal{Z}_{p}$ \cite{reimers2019sentence}. %A single encoded passage in $\mathcal{Z}_{\mathbf{P}}$ is represented as $z_{P}$.
% Likewise, encoding of $k_d$ is represented as $\mathcal{Z}_{k_d}$. 
% The algorithm used for ranked passage retrieval is SITQ(Simple local sensitive hashing (Simple-LSH) and Iterative Quantization). SITQ retrieval and ranking can be formalized as $Score(\mathbf{P}_{\mbox{top-K}}|k_d)$ where 

==> results.tex <==
\begin{table*}[!htbp]
\scalebox{0.8}{
{\fontfamily{cmss}\selectfont
\begin{tabular}{p{3.2cm}p{1.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.5cm}p{0.8cm}|p{0.7cm}p{0.7cm}p{0.7cm}p{0.5cm}p{0.8cm}|p{0.7cm}p{0.7cm}p{0.7cm}p{0.5cm}p{0.8cm}}
\toprule[1.5pt]
\textbf{Methods} & \textbf{SQE} & \multicolumn{5}{c}{\textbf{QADiscourse}} & \multicolumn{5}{c}{\textbf{QAMR}} & \multicolumn{5}{c}{\textbf{FB Curiosity}} \\ 
& & R-L & BRT & BScore & SR & LC(\%) & R-L & BRT & BScore & SR & LC(\%) & R-L & BRT & BScore & SR & LC(\%) \\ \toprule[1.5pt]
\multirow{3}{*}{T5-FT WikiPassageQA} & - & 0.37 & 0.43 & 0.16 & 0.17 & 10.0 & 0.19 & 0.51 & 0.38 & 0.36 & 17.0 
& 0.65 & 0.78 & 0.54 & 0.51 & 47.3 \\
& +\textcolor{OliveGreen}{Entities} & 0.39 & 0.45 & 0.16 & 0.17 & 10.0 & 0.20 & 0.53 & 0.38 & 0.36 & 17.5 
& 0.65 & 0.78 & 0.54 & 0.52 & 47.4 \\  
 & +\textcolor{blue}{Triples}& 0.41 & 0.46 & 0.16 & 0.18 & 11.0 & 0.2 & 0.53 & 0.39 & 0.37 & 17.8 &  
0.65 & 0.78 & 0.55  & 0.52 & 47.3 \\ \cmidrule{2-17}
\multirow{3}{*}{T5-FT SQUAD} & - & 0.44 & 0.54 & 0.20 & 0.19& 13.0 & 0.40 & 0.66 & 0.46 & 0.58 & 21.0 
& 0.70 & 0.83 & 0.62 & 0.67 & 65.1\\ 
& +\textcolor{OliveGreen}{Entities} & 0.45 & 0.56 & 0.22 & 0.19 & 13.5 & 0.40 & 0.68 & 0.47 & 0.59 & 22.7 
& 0.71 & 0.84 & 0.63 & 0.69 & 65.8 \\ 
 & +\textcolor{blue}{Triples} & 0.45 & 0.58 & 0.22 & 0.20 & 13.8 & 0.43 & 0.69 & 0.47 & 0.59 & 22.6  
& 0.70 & 0.84 & 0.64 & 0.69 & 65.8 \\ \cmidrule{2-17}
\multirow{3}{*}{T5-FT CANARD} & - & 0.47 & 0.54 & 0.23 & 0.19 & 17.1 & 0.41 & 0.64 & 0.53 & 0.58 & 22.6 
& 0.73 & 0.84 & 0.63 & 0.67 & 66.2 \\
& +\textcolor{OliveGreen}{Entities} & 0.48 & 0.55 & 0.25 & 0.20 & 17.5 & 0.44 & 0.67 & 0.62 & 0.61 & 23.5 
& 0.74 & 0.84 & 0.65 & 0.69 & 66.5 \\
& +\textcolor{blue}{Triples} & 0.51 & 0.57 & 0.26 & 0.21 & 18.3 & 0.49 & 0.68 & 0.66 & 0.61 & 24.3 
& 0.74 & 0.85 & 0.65 & 0.70 & 68.2 \\ \cmidrule{2-17}
\multirow{3}{*}{ProphetNet-FT SQUAD} &-& 0.24 & 0.38 & 0.11 & 0.17 & 11.0 & 0.23 & 0.61 & 0.39 & 0.37 & 17.7 
& 0.56 & 0.68 & 0.51 & 0.60 & 57.3 \\
& +\textcolor{OliveGreen}{Entities} & 0.26 & 0.39 & 0.13 & 0.17 & 11.0 & 0.29 & 0.62 & 0.41 & 0.37 & 18.1 
& 0.58 & 0.70 & 0.51 & 0.62 & 58.4 \\
& +\textcolor{blue}{Triples} & 0.27 & 0.41 & 0.17 & 0.17 & 11.0 & 0.34 & 0.65 & 0.43 & 0.38 & 19.0 
& 0.58 & 0.72 & 0.50 & 0.63 & 59.7 \\ \cmidrule{2-17}
\multirow{3}{*}{Electra-FT SQUAD} &-& 0.31 & 0.44 & 0.14 & 0.17 & 12.2 & 0.35 & 0.59 & 0.38 & 0.36 & 21.5 
& 0.63 & 0.78 & 0.53 & 0.67 & 63.2 \\
 & +\textcolor{OliveGreen}{Entities} & 0.31 & 0.44 & 0.14 & 0.17 & 12.7 & 0.37 & 0.60 & 0.41 & 0.37 & 22.1 
& 0.65 & 0.78 & 0.54 & 0.67 & 63.3 \\
& +\textcolor{blue}{Triples} & 0.34 & 0.45 & 0.15 & 0.18 & 13.0 & 0.37 & 0.61 & 0.43 & 0.37 & 22.3 
& 0.65 & 0.79 & 0.56 & 0.69 & 64.0 \\ \bottomrule[1.2pt]
%\multicolumn{17}{c}{\textbf{Proposed Approach}} \\ \bottomrule[1pt]
\multirow{3}{*}{{\fontfamily{cmss}\selectfont ISEEQ-RL}} & - & 0.57 & 0.72 & 0.40 & 0.22 & 20.0 & 0.50 & 0.75 & 0.67 & 0.64 & 29.4 & 0.71 & 0.84 &0.62 & 0.69 & 68.2  \\
& +\textcolor{OliveGreen}{Entities} & 0.64 & 0.72 & 0.41 & 0.23 & 22.0 & 0.52 & 0.77 & 0.68 & 0.64 & 33.1 & 0.72 & 0.85 & 0.63 & 0.71 & 69.8 \\
& +\textcolor{blue}{Triples} & 0.65 & 0.74 & 0.45 & 0.25 & 22.0 & 0.53 & 0.78 & 0.71 & 0.65 & 34.7 &0.74 & 0.87 & 0.63 &0.73 &71.8 \\ \cmidrule{2-17}
\multirow{3}{*}{{\fontfamily{cmss}\selectfont ISEEQ-ERL}} & - & 0.60 & 0.76 & 0.44 & 0.26 & 24.5 & 0.55 & 0.81 & 0.72 & 0.68 & 36.1 
&0.74 & 0.85 & 0.64 & 0.76 & 78.2 \\
& +\textcolor{OliveGreen}{Entities} & 0.65 & 0.78 & 0.47 & 0.27 & 25.2 & 0.55 & 0.82 & 0.74 & 0.68 & 36.3 
& 0.77 & 0.88 & 0.66 & 0.76 & 78.3 \\
& +\textcolor{blue}{Triples} & \textbf{0.67} & \textbf{0.79} & \textbf{0.50} & \textbf{0.27} & \textbf{25.7} & \textbf{0.57} & \textbf{0.83} & \textbf{0.77} & \textbf{0.68} & \textbf{37.0} & \textbf{0.79} & \textbf{0.89} & \textbf{0.66} & \textbf{0.78} & \textbf{79.4}\\
\bottomrule[1.5pt]
\end{tabular}}}
\caption{\footnotesize Test scores of baselines and proposed approach on discourse datasets. Compared to T5-FT CANARD, {\fontfamily{cmss}\selectfont ISEEQ-ERL} generated better questions across three datasets (30\%$\uparrow$ in QADiscourse, 7\%$\uparrow$ in QAMR, and 5\%$\uparrow$ in FB Curiosity).}
\label{tab:major_results}
\end{table*}


\begin{table}[!htbp]
    \scriptsize
    \begin{tabular}{p{1.cm}|p{1.4cm}|p{1.4cm}|p{1.4cm}|p{1.4cm}}
    \toprule[1.5pt]
    \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Encoding}} & \textbf{QAD} & \textbf{QAMR} & \textbf{FBC} \\ \cmidrule{3-5}
    & & \multicolumn{3}{c}{R-L/BRT/BScore/SR/LA} \\ \midrule[1pt]
    \multirow{2}{*}{{\fontfamily{cmss}\selectfont ISEEQ-RL}} & \textcolor{Fuchsia}{$P_{1:K}$} & 0.62/ 0.73/ 0.39/ 0.21/ 21.3 & 0.47/ 0.71/ 0.39/ 0.63/ 28 & 0.74/ 0.83/ 0.60/ 0.73/ 71.6 \\ \cmidrule{3-5}              
       & \textcolor{NavyBlue}{$P_{1:K}$+ SQE} & 0.65/ 0.74/ 0.45/ 0.25/ 22 & 0.53/ 0.78/ 0.71/ 0.65/ 34.7 & 0.74/ 0.87/ 0.65/ 0.73/ 71.8\\ \midrule[1pt]
    \multirow{2}{*}{{\fontfamily{cmss}\selectfont ISEEQ-ERL}} & \textcolor{Fuchsia}{$P_{1:K}$} & 0.62/ 0.76/ 0.44/ 0.26/ 24.6 & 0.54/ 0.80/ 0.73/ 0.68/ 36.3 & 0.71/ 0.84/ 0.61/ 0.77/ 78.2 \\\cmidrule{3-5}
    & \textcolor{NavyBlue}{$P_{1:K}$+ SQE} & 0.67/ 0.79/ 0.50/ 0.27/ 25.7 &0.57/ 0.83/ 0.77/ 0.68/ 37.0 & 0.79/ 0.89/ 0.66/ 0.78/ 79.4 \\ \bottomrule[1.5pt]
    \end{tabular}
    \caption{\footnotesize Ablation study on encoding the retrieved passage ($\mathbf{P}_{1:K}$)and query expansion (SQE) for QG.}
    \label{tab:ablation}
\end{table}


\paragraph{Performance of {\fontfamily{cmss}\selectfont ISEEQ-RL} and {\fontfamily{cmss}\selectfont ISEEQ-ERL} :}
Table \ref{tab:major_results} shows that infusion of knowledge in queries significantly improves natural language question generation in open domain. Particularly in  T5-FT CANARD, which stood out as the most competitive baseline. It is because of the question-in-context rewriting capability that focuses on syntactic and semantic consistency. However, it is not aware of semantic relations and logical coherence in question generation. Thus, {\fontfamily{cmss}\selectfont ISEEQ-ERL} significantly outperformed T5-FT CANARD and other baselines by large margins across all the five metrics. Even {\fontfamily{cmss}\selectfont ISEEQ-RL} without SQE equals T5-FT CANARD. Furthermore, it shows that retrieval of multiple relevant passages by KPR surpassed single passage TLMs, often considered in prior works in CIS. 
Most of the CAsT-19 and FB Curiosity (FBC) queries required multiple passages to construct legible questions. For instance, Is-type question: ``Enquiry about History, Economy, and Sports in Hyderabad'' requires three passages on ``History\_Hyderabad'', ``Economy\_Hyderabad'', and ``Sports\_Hyderabad'' which were missing in gold passages. Thus, TLM-FT baselines find it hard to construct legible Is-type questions using the gold passage. {\fontfamily{cmss}\selectfont ISEEQ-RL} and {\fontfamily{cmss}\selectfont ISEEQ-ERL} prevented the loss by finding answers in passages that share semantic relations to gold passages. It showed that models generated legible questions that have semantic relations and logical coherence with ground truth. Ablations on encodings were performed to experiment separate contributions of KPR ($\mathbf{P}_{1:K}$) and SQE in question generation. Table \ref{tab:ablation} records an average improvement of 2-6\% across all discourse datasets.

\begin{table}[!htbp]
{\fontfamily{cmss}\selectfont
\footnotesize
\begin{tabular}{c|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}}
        \toprule[1.5pt]
         \textbf{Ret.Pass.} & \multicolumn{2}{c}{\textbf{DPR}} & \multicolumn{2}{c}{\textbf{KPR-E}} & \multicolumn{2}{c}{\textbf{KPR-ET}}  \\ 
         & Train & Test & Train & Test & Train & Test \\ \midrule[1pt]
         5K & 71 & 123 & 99 & 278 & 157 & 275 \\
         10K & 96 & 133 & 154 & 301 & 194 & 316 \\
         25K & 139 & 133 & 235 & 329 & 236 & 363 \\
         50K & 173 & 144 & \textbf{269} & 358 & \textbf{269} & \textbf{402} \\ \bottomrule[1.5pt]
    \end{tabular}}
    \caption{\footnotesize Retrieving passages from MS-MARCO for CAsT-19.}
    \label{tab:cast19_1}
\end{table}

\begin{figure}[!htbp]
{\fontfamily{cmss}\selectfont
\begin{minipage}[h]{1.0\linewidth}
\centering
\subfloat[][]{\resizebox{0.5\textwidth}{!}{
\begin{tikzpicture}
\begin{axis}[legend style={nodes={scale=0.5, transform shape}}, width=7.5cm, height=4.5cm,
    ybar,
    bar width=5pt,
    xlabel={Retrieved Passages},
    ylabel={Semantic Relations},
    xtick=data,
    xticklabels from table={\datatable}{A},
    ymajorgrids,
    legend pos=north west
             ]
    \addplot table [x expr=\coordindex, y= B]{\datatable};
    \addplot table [x expr=\coordindex, y= C]{\datatable};
    \addplot table [x expr=\coordindex, y= D]{\datatable};
    \addplot table [x expr=\coordindex, y= E]{\datatable};
    \legend{Baseline,{\fontfamily{cmss}\selectfont ISEEQ-RL},(KPR-E)+{\fontfamily{cmss}\selectfont ISEEQ-RL}, (KPR-ET)+{\fontfamily{cmss}\selectfont ISEEQ-RL}}
\end{axis}
\end{tikzpicture}}}
\subfloat[][]{\resizebox{0.5\textwidth}{!}{
\begin{tikzpicture}
\begin{axis}[legend style={nodes={scale=0.5, transform shape}}, width=7.5cm, height=4.5cm,
    ybar,
    bar width=5pt,
    xlabel={Retrieved Passages},
    ylabel={Logical Coherence},
    xtick=data,
    xticklabels from table={\datatables}{A},
    ymajorgrids,
    legend pos=north west
             ]
    \addplot table [x expr=\coordindex, y= B]{\datatables};
    \addplot table [x expr=\coordindex, y= C]{\datatables};
    \addplot table [x expr=\coordindex, y= D]{\datatables};
    \addplot table [x expr=\coordindex, y= E]{\datatables};
    \legend{Baseline,{\fontfamily{cmss}\selectfont ISEEQ-RL},(KPR-E)+{\fontfamily{cmss}\selectfont ISEEQ-RL}, (KPR-ET)+{\fontfamily{cmss}\selectfont ISEEQ-RL}}
\end{axis}
\end{tikzpicture}}}
\end{minipage}
%--------------------------------
\begin{minipage}[h]{1.0\linewidth}
\centering
\subfloat[][]{\resizebox{0.5\textwidth}{!}{
\begin{tikzpicture}
\begin{axis}[legend style={nodes={scale=0.5, transform shape}}, width=7.5cm, height=4.5cm,
    ybar,
    bar width=5pt,
    xlabel={Retrieved Passages},
    ylabel={Semantic Relations},
    xtick=data,
    xticklabels from table={\datatabless}{A},
    ymajorgrids,
    legend pos=north west
             ]
    \addplot table [x expr=\coordindex, y= B]{\datatabless};
    \addplot table [x expr=\coordindex, y= C]{\datatabless};
    \addplot table [x expr=\coordindex, y= D]{\datatabless};
    \addplot table [x expr=\coordindex, y= E]{\datatabless};
    \legend{(KPR-E)+{\fontfamily{cmss}\selectfont ISEEQ-RL},(KPR-E)+{\fontfamily{cmss}\selectfont ISEEQ-ERL},(KPR-ET)+{\fontfamily{cmss}\selectfont ISEEQ-RL}, (KPR-ET)+{\fontfamily{cmss}\selectfont ISEEQ-ERL}}
\end{axis}
\end{tikzpicture}}}
\subfloat[][]{\resizebox{0.5\textwidth}{!}{
\begin{tikzpicture}
\begin{axis}[legend style={nodes={scale=0.5, transform shape}}, width=7.5cm, height=4.5cm,
    ybar,
    bar width=5pt,
    xlabel={Retrieved Passages},
    ylabel={Logical Coherence},
    xtick=data,
    xticklabels from table={\datatablesss}{A},
    ymajorgrids,
    legend pos=north west
             ]
    \addplot table [x expr=\coordindex, y= B]{\datatablesss};
    \addplot table [x expr=\coordindex, y= C]{\datatablesss};
    \addplot table [x expr=\coordindex, y= D]{\datatablesss};
    \addplot table [x expr=\coordindex, y= E]{\datatablesss};
    \legend{(KPR-E)+{\fontfamily{cmss}\selectfont ISEEQ-RL},(KPR-E)+{\fontfamily{cmss}\selectfont ISEEQ-ERL},(KPR-ET)+{\fontfamily{cmss}\selectfont ISEEQ-RL}, (KPR-ET)+{\fontfamily{cmss}\selectfont ISEEQ-ERL}}
\end{axis}
\end{tikzpicture}}}
\end{minipage}}
\caption{\footnotesize (a) and (b): Generation scores of the pipeline: KPR-(E,ET) combined with {\fontfamily{cmss}\selectfont ISEEQ-RL} and {\fontfamily{cmss}\selectfont ISEEQ-ERL} on CAsT-19 Dataset. (c) and (d): Substantial improvement in generations because of entailment loss in {\fontfamily{cmss}\selectfont ISEEQ-ERL}. Baseline: T5-FT CANARD.}  
\label{fig:cast19_results}
\end{figure}


\paragraph{Performance of KPR + {\fontfamily{cmss}\selectfont ISEEQ-ERL}:} CAsT-19 presents a unique real-world challenge in terms of diverse context and semantic phenomena on a small dataset. Experiments on CAsT-19 assessed the combined utility of KPR and {\fontfamily{cmss}\selectfont ISEEQ-ERL}. For each input query, in any iteration of KPR, top-100 passages were retrieved and checked for the presence of $>$80\% of the entities (exact match). KPR is stopped after each query in the train set has at least one passage. With $\sim$50K passages KPR fulfilled to task compared to DPR. Further, KPR-E and KPR-ET retrieved passages for 75\% and 84\% of input queries in the CAsT-19 test, respectively. Whereas DPR support 30\% queries in train set (see Table \ref{tab:cast19_1}). Figure \ref{fig:cast19_results} (a) illustrates the quality of {\fontfamily{cmss}\selectfont ISEEQ-RL} generations on the CAsT-19 dataset, which are 27\% more semantic similar and related with the ground truth compared to T5-FT CANARD. {\fontfamily{cmss}\selectfont ISEEQ-RL} with SQE generated 54\% questions that entail a ground truth question in CAsT-19\footnote{it means of 10 generated questions, 5 or 6 can be logically inferred from ground truth question} (Figure \ref{fig:cast19_results}(b).(KPR-E)+{\fontfamily{cmss}\selectfont ISEEQ-ERL} and (KPR)-ET+{\fontfamily{cmss}\selectfont ISEEQ-ERL} seems to generate Is-type questions with significantly large logical coherence and concept flow. Moreover, figure \ref{fig:cast19_results}(c,d) illustrates the remarkable improvement in the generation of questions with the conceptual flow with a lower number of retrieved passages on a highly complex CAsT-19 dataset. We attribute this to the addition of loss function optimizers: entailment probability and RCE.


\begin{table}[!ht]
\scriptsize
\scalebox{0.9}{
{\fontfamily{cmss}\selectfont
\begin{tabular}{p{1cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}
\toprule[1.5pt]
&  \textbf{QAD} & \textbf{QAMR}  & \textbf{FBC} & \textbf{CAsT19} \\ \cmidrule{2-5}
& \multicolumn{3}{c}{R-L/BRT/BScore/SR/LC(\%)} \\ \midrule[1pt] 
\textbf{QAD} & \textbf{0.67/ 0.79/ 0.50/ 0.27/ 25.7} & 0.56/ 0.79/ 0.75/ 0.64/ 33.1 & 0.62/ 0.70/ 0.55/ 0.71/ 73.5 & 0.76/ 0.48/ 0.64/ 0.60/ 64.2\\
\textbf{QAMR} & 0.73/ 0.89/ 0.62/ 0.28/ 27.7 & \textbf{0.57/ 0.83/ 0.77/ 0.68/ 37.0} & 0.74/ 0.89/ 0.67/ 0.75/ 77.8 & 0.67/ 0.41/ 0.57/ 0.57/ 58.6\\
\textbf{FBC} & 0.70/ 0.73/ 0.56/ 0.31/ 33.0 & 0.61/ 0.85/ 0.72/ 0.67/ 35.8 & \textbf{0.79/ 0.89/ 0.66/ 0.78/ 79.4} & 0.75/ 0.37/ 0.76/ 0.67/ 66.5 \\
\textbf{CAsT-19} & 0.58/ 0.69/ 0.51/ 0.23/ 25.2 & 0.52/ 0.73/ 0.70/ 0.61/ 33.4 & 0.63/ 0.77/ 0.57/ 0.73/ 76.5 & \textbf{0.74/ 0.48/ 0.68/ 0.61/ 65.0} \\ \bottomrule[1.5pt]
\end{tabular}}}
\caption{\footnotesize Domain-Adaptation test scores using M2\_RQREL (Read By Row: M2\_RQREL was train on QAD) and tested on QAD, QAMR, and FBC). Bold-Faced: M2\_RQREL was trained and tested on same dataset.}
\label{tab:domain_1}
\end{table}

\paragraph{Domain Adaptation:} {\fontfamily{cmss}\selectfont ISEEQ-ERL} is trained and tested on datasets covering different domains. For instance, training on QADiscourse, which covers articles from WikiNews, and testing on CAsT-19 covering articles from the web (science, health, history, etc.). Performance scores on five metrics examine the generalizability of {\fontfamily{cmss}\selectfont ISEEQ-ERL}. Table \ref{tab:domain_1} records improvement in IsQG in CAsT-19 by 2\% on R-L, 6\% on BScore, 2\% on SR, and 1.2\% on LC after M2\_RQREL was trained on QAD. Further, training {\fontfamily{cmss}\selectfont ISEEQ-ERL} on QAMR presented results on the FBC test set comparable to the experiment involving train-test on FBC. Likewise, training {\fontfamily{cmss}\selectfont ISEEQ-ERL} on QAD and testing on QAMR presented results which are close to train-test on QAMR\footnote{we tested overlap between retrieved passages in QAD, QAMR, FBC, and CAsT-19. They showed statistical difference with p-value<0.02}. 

\begin{table}[!ht]
\footnotesize 
\scalebox{0.9}{
{\fontfamily{cmss}\selectfont
\begin{tabular}{p{1.cm}p{2cm}p{2cm}p{2cm}}
\toprule[1.5pt]
&  \textbf{S1\&S2} & \textbf{S1\&S3}  & \textbf{S2\&S3} \\
G1 & S1==S2 (p$>$0.1) & S1==S3 (p$>$0.1) & S2$>$S3 (p$<$0.1,wp=0.0015) \\
G2 & S1==S2 (p$>$0.1)	& S1$>$S3 (p$<$0.1, wp=0.03) & S2$>$S3 (p$<$0.1,wp=0.003) \\
G3 & S2$>$S1(p$<$0.1, wp=3.46E-06) & S1$>$S3 (p<0.1, wp=1.58E-05) & S2>S3 (p$<$0.1, wp=0.0008) \\
G4 & S2$>$S1(p$<$0.1, wp=0.04) & S1$>$S3 (p$<$0.1, wp=3.57E-14)	& S2>S3(p$<$0.1, wp=2.03E-10) \\
G5 & S1==S2 (p$>$0.1) & S1$>$S3 (p$<$0.1, wp=1.72E-08) & S2$>$S3(p<0.1, wp=0.09) \\
\bottomrule[1.5pt]
\end{tabular}}}
\caption{\footnotesize Evaluating IS-type QG systems on 5 guidelines. For both ANOVA and Wilcoxon, statistical significance was measured at p-value(p)$<$ 0.1 and wilcoxon p-value (wp) $<$ 0.1. }
\label{tab:human_eval}
\end{table}

\paragraph{Human Evaluation:} We carried out ten blind evaluations\footnote{users didn't know which system generated IS-type questions} to see how users rate generated questions along five guidelines (G) created using qualitative studies in CIS:
G1: Are the questions in a well-formed English language; G2: Are the questions rich in gathering relevant context?; G3: Are the questions diverse and non-redundant?; G4 Are the question logically coherent?; and G5: Will answers to these questions satisfy the user's information needs? Each of these questions got integer scores between 1 (low) to 5 (high). Each human evaluation comprises 30 user queries covering domains such as Health, Science, History, Geography. On average, system 1 (S1: Ground Truth), system 2 (S2: ISEEQ-ERL), and system 3 (S3: T5-FT CANARD) generated 7, 7, 5 questions per query. All the evaluators were allowed to use web resources for side information on queries to perform high-quality assessments. We examined the ratings of systems on G1-G5 for variance using one-way ANOVA. If a pair of systems, for instance, S1\&S2, receive ratings on G1 with no significant variance, we consider these systems to be similar in performance on G1. On the other hand, if there is a statistically significant difference, we perform a one-tailed Wilcoxon signed-rank test\footnote{define wilcoxon} to see which system gained confidence in evaluators. From Table \ref{tab:human_eval}, we make following interpretations: \textbf{(1)} For G1, there was a significant variance in ratings between S2\&S3, with evaluators' findings S2 generated questions to be more legible than S3. However, S1\&S2 and S1\&S3 had ratings with marginal variations. \textbf{(2)} G2, G3, and G4 evaluations suggested S2 effectively contextual information gathering over S1 and S3. This also addresses \textbf{RQ2} that emphasizes logical coherence and semantic relations for efficient CIS. \textbf{(3)} G5 mainly ask evaluators, ``Which system would they pick for addressing their information needs?'' and we found them selecting S1 and S2 in the majority. However, based on our feedback, for a few complex queries, such as ``Need help. Bothered by little interest or pleasure in doing things'', ''Need to know about Gemini VIII. Armstrong used an emergency set of thrusters to regain control. Gemini VIII landed in the Pacific Ocean after ten hours of flight''; they were indecisive between S2 and S3, giving them the same ratings (wp=0.09 $<$ 0.1).
